Pangu-Agent: A Fine-Tunable Generalist Agent with Structured Reasoning

A key method for creating Artificial Intelligence (AI) agents is Reinforcement Learning (RL). However, constructing a standalone RL policy that maps perception to action directly encounters severe problems, chief among them being its lack of generality across multiple tasks and the need for a large amount of training data. The leading cause is that it cannot effectively integrate prior information into the perception-action cycle when devising the policy. Large language models (LLMs) emerged as a fundamental way to incorporate cross-domain knowledge into AI agents but lack crucial learning and adaptation toward specific decision problems. This paper presents a general framework model for integrating and learning structured reasoning into AI agents' policies. Our methodology is motivated by the modularity found in the human brain. The framework utilises the construction of intrinsic and extrinsic functions to add previous understandings of reasoning structures. It also provides the adaptive ability to learn models inside every module or function, consistent with the modular structure of cognitive processes. We describe the framework in-depth and compare it with other AI pipelines and existing frameworks. The paper explores practical applications, covering experiments that show the effectiveness of our method. Our results indicate that AI agents perform and adapt far better when organised reasoning and prior knowledge are embedded. This opens the door to more resilient and general AI agent systems.

==> models.tex <==
\begin{itemize}
    \item \href{https://huggingface.co/tiiuae/falcon-7b-instruct}{tiiuae/falcon-7b-instruct · Hugging Face}
    \item \href{https://huggingface.co/Intel/neural-chat-7b-v3-1}{Intel/neural-chat-7b-v3-1 · Hugging Face} 
    \item \href{https://huggingface.co/nvidia/nemotron-3-8b-chat-4k-rlhf}{nvidia/nemotron-3-8b-chat-4k-rlhf · Hugging Face} 
    \item \href{https://huggingface.co/vivo-ai/BlueLM-7B-Chat-32K}{vivo-ai/BlueLM-7B-Chat-32K · Hugging Face} 
    \item \href{https://huggingface.co/TheBloke/Nanbeige-16B-Chat-32K-GGUF}{TheBloke/Nanbeige-16B-Chat-32K-GGUF · Hugging Face} 
    \end{itemize}

==> paper/0-front.tex <==
\paragraph{Copyright Huawei Technologies Co., Ltd. 2022. All rights reserved.} \quad\\
No part of this document may be reproduced or transmitted in any form or by any means without prior written consent of Huawei Technologies Co., Ltd.

\paragraph{Trademarks and Permissions} \quad\\
\includegraphics[width=0.05\linewidth]{figures/huawei.png} and other Huawei trademarks are trademarks of Huawei Technologies Co., Ltd.
All other trademarks and trade names mentioned in this document are the property of their respective holders.

\paragraph{Notice} \quad\\
The purchased products, services and features are stipulated by the contract made between Huawei and the customer. All or part of the products, services and features described in this document may not be within the purchase scope or the usage scope. Unless otherwise specified in the contract, all statements, information, and recommendations in this document are provided "AS IS" without warranties, guarantees or representations of any kind, either express or implied.


The information in this document is subject to change without notice. Every effort has been made in the preparation of this document to ensure accuracy of the contents, but all statements, information, and recommendations in this document do not constitute a warranty of any kind, express or implied.
~\\[100pt]


\begin{LARGE}
Huawei Technologies Co., Ltd.
\end{LARGE}

~\\[5pt]
\begin{tabular}{cl}
     Address: & Huawei Industrial Base \\
              & Bantian, Longgang \\
              & Shenzhen 518129 \\
              & People's Republic of China \\
     Website: & http://www.huawei.com/
\end{tabular}


==> paper/2-related.tex <==
\section{Related Work}
\label{sec:related}

Auto-GPT, LangChain, XLANG Agent, BabyAGI, TPTU, auto-Agent

\subsection{Chain-of-Thought (COT)}

Chain of Thought prompting is one of the most popular prompting technique to improve the reasoning capabilities of language models. It was first introduced in \citep{wei2022chain} as a series of intermediate reasoning steps to improve complex reasoning abilities in language models, where a few CoT examples are provided to the model to learn from. There are many such methods stemming from it.

Tree of Thoughts \citep{yao2023tree} allows for the exploration over coherent units of thoughts by allowing models to make decisions by considering multiple reasoning directions and self-evaluating its choices. Active-Prompting with CoT \citep{diao2023active} is a technique in which examples are annotated with human-designed CoT, on those examples for which the model is most uncertain (which is checked through asking the model its level of certainty of a response). Least-to-Most prompting \citep{zhou2023leasttomost} looks to break down a complex reasoning task into sub-tasks in order to allow the agent to solve them sequentially. Each sub-task is provided with previously solved sub-tasks as context for the model. Another modification of CoT is Graph-of-Thought (GoT) reasoning \citep{yao2023beyond} which explores having not just chain, but graphs with thought units as nodes and connections between thoughts as edges. It proposes to mimic a more human-like thinking process which is non-sequential. Iteratively Prompting LLMs for CoT is a technique in which the prompts are dynamically synthesized based on the current step's contexts. Zero-shot CoT \citep{NEURIPS2022_8bb0d291} is another method in which no prior CoT examples are given to the model, but the model is simply prompted to "think step-by-step" at the end of the question. This technique can generalise over an array of tasks and allows the agent to use reasoning capabilities to improve response accuracy.

\subsection{Single-Agent}
The rapid advancement in the general capabilities of large language models has catalyzed the development of more complex and capable LLM-based agents, across both text-based and multimodal environments.

A range of proof-of-concept works have demonstrated the reasoning and planning abilities of large language models. Works such as Chain-of-Thought\citep{wei2022chain}, Self Consistency\citep{wang2022self}, Tree of Thoughts\citep{yao2023tree,long2023large}, and Graph of Thoughts\citep{yao2023beyond,besta2023graph} exhibit models' aptitude for structured conceptual exploration. Other efforts emphasize the iterative self-improvement capacities of LLMs, including Self-Refine\citep{madaan2023self}, ReAct\citep{yao2022react}, ReWOO\citep{xu2023rewoo}, Reflexion\citep{shinn2023reflexion}, and Chain-of-Hindsight \citep{liu2023languages}. These works provide existence proofs that LLMs have the basic underlying capacity to support reasoning, planning, memory, and iterative self-improvement needed for capable agents.



Other efforts have focused on developing agent frameworks to enable LLMs to tackle more complex settings. Single-agent frameworks incorporate the LLM as a central controller alongside other modular components. ( Actually I think there is not a clear decision boundary between the conception of the agent (depending on LLM or not) and some sophisticated tool component, as sometimes the functionality of a LLM backed agent is more like a LLM enhanced tool) For example, the GPT-4\citep{openai2023gpt4} model on the OpenAI platform can serve as a personal assistant agent, leveraging plugins, code interpreter and web integration to operate in closed and open environments. Open Interpreter\citep{openinterpreter} and OpenAgents\citep{xie2023openagents} is an open-source implementation trying to emulate the agent structure on the Openai platform. Transformer Agents\citep{wolf2019huggingface} and LangChain\citep{LangChain} are open-source repositories been developed to help developers to build single LLM agent more easily with built-in functionalities. AutoGPT\citep{autogpt2023} focuses on utilizing LLM for achieving flexible goals within a single agent structure. Other proposed single-agent frameworks like Gentopia\citep{xu2023gentopia}, AgentGPT\citep{agentgpt} follow similar ideas like AutoGPT.


\subsection{Multi-Agent}
To unlock more advanced features required for complex tasks, multi-agent frameworks have been explored. While preliminary works like Camel\citep{li2023camel}, Multi-Agent Debate\citep{liang2023encouraging,du2023improving}, BabyAGI\citep{babyagi}, CHATDEV\citep{qian2023communicative}, MetaGPT\citep{hong2023metagpt}, RestGPT\citep{song2023restgpt}, ProAgent\citep{zhang2023proagent} demonstrate the potential for multiple LLMs to collaborate on challenges difficult for a single agent, their communication patterns between agents are relatively fixed.

More recent work has focused on making multi-agent communication more flexible. BOLAA\citep{liu2023bolaa} utilizes a controller module to manage communication between "labor" agents. AgentVerse\citep{chen2023agentverse} combines expert recruitment with collaborative decision-making to adapt to different tasks. AutoAgents\citep{chen2023auto} employs observer agents to enhance recruitment, collaboration, and action execution process. Dylan\citep{liu2023dynamic} 
 enable dynamic multi-agent architecture and automatic agent team optimization. Some frameworks further emphasize customizability and extensibility. Configurability is a shared feature among these frameworks.  AGENTS\citep{zhou2023agents} uses configurable symbolic plans called Standard Operating Procedures to control agent behaviors. AutoGen\citep{wu2023autogen} focuses on customizable Conversable Agents and Conversation Programming to enable flexible conversation patterns between agents for collaborative reasoning. 
 
\subsection{World Model}

To further improve the language model agent in the long-horizon decision-making problems, some research has implement the "world model" in the reasoning process. The basic idea is that human have inherent understanding of the environment and can predict the future events without interaction with real world. \citep{liu2023reason} \citep{hao2023reasoning}


%I think our framework has some advantages over previous frameworks:

%1. Although frameworks like Autogen and AGENTS both implement configurable initialization of parameters. Pangu-agent will enable more comprehensive customizability. (Memory and Prompting Techniques in Figure 1; switching modules on and off;) 

%2. The iterative thinking process enables more general self-improvement of agent components than previous works.

%3. More prompting techniques are integrated into the framework



==> paper/4-evaluation.tex <==
\section{Agent Evaluation}
\label{sec:evaluation}


\subsection{AgentBench, WebArena, GSM8K, HotpotAQ, MA taks (software developments)}

Prompt optimization \textcolor{red}{Thomas Coste, Jingxuan Chen, Zhihao Wu, Khyati Khandelwa}

Finetuning \textcolor{red}{Matthiue, Jonas}



==> paper/5-application.tex <==
\section{Applications}
\label{sec:applications}
Potential applications, including personal assistant, robotics, EDA, and so on.

% \subsection{Personal Assistant \textcolor{red}{CBG Xiaoyi team,  GTS team (Zhenghua Dong \& Qiang Ye)}}

% \subsection{Robotics \textcolor{red}{(Matthieu \& Guangjian Tian \& Peng Du)}}

% \subsection{EDA \textcolor{red}{(Mingxuan's team)}}

==> test_table.tex <==

\begin{table}[ht]
\centering
\begin{tabular}{lrrrrrrr}
\toprule
Method & Overall & ALFWorld & GSM8K & HotpotQA & Webshop & Humaneval & BabyAI \\
direct & 6.5 & 4.0 \small{$ \pm \ 1.6$} & 14.1 \small{$ \pm \ 0.7$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 7.7 \small{$ \pm \ 3.2$} \\
zs-cot & 15.2 & 9.3 \small{$ \pm \ 3.8$} & 33.9 \small{$ \pm \ 0.7$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 17.4 \small{$ \pm \ 4.4$} \\
fs & 3.1 & 6.0 \small{$ \pm \ 1.6$} & 0.5 \small{$ \pm \ 0.0$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 6.0 \small{$ \pm \ 3.3$} \\
fs-cot & 16.8 & 6.0 \small{$ \pm \ 0.0$} & 32.7 \small{$ \pm \ 0.3$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 28.6 \small{$ \pm \ 3.9$} \\
fs-cot-sc & 20.9 & N/A & 38.2 \small{$ \pm \ 0.7$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 24.4 \small{$ \pm \ 3.3$} \\
fs-cot-react & 9.3 & N/A & 19.9 \small{$ \pm \ 1.1$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 7.9 \small{$ \pm \ 2.0$} \\
fs-cot-reflect & 7.8 & N/A & 0.0 \small{$ \pm \ 0.0$} & N/A & N/A & 0.0 \small{$ \pm \ 0.0$} & 23.3 \small{$ \pm \ 2.5$} \\
fs-least2most & nan & N/A & N/A & N/A & N/A & N/A & N/A \\

\midrule\end{tabular}\end{table}
